Counterfactual Gradients-based Quantification of Prediction Trust in Neural Networks

The widespread adoption of deep neural networks in machine learning calls for an objective quantification of esoteric trust. In this paper we propose GradTrust, a classification trust measure for large-scale neural networks at inference. The proposed method utilizes variance of counterfactual gradients, i.e. the required changes in the network parameters if the label were different. We show that GradTrust is superior to existing techniques for detecting misprediction rates on $50000$ images from ImageNet validation dataset. Depending on the network, GradTrust detects images where either the ground truth is incorrect or ambiguous, or the classes are co-occurring. We extend GradTrust to Video Action Recognition on Kinetics-400 dataset. We showcase results on $14$ architectures pretrained on ImageNet and $5$ architectures pretrained on Kinetics-400. We observe the following: (i) simple methodologies like negative log likelihood and margin classifiers outperform state-of-the-art uncertainty and out-of-distribution detection techniques for misprediction rates, and (ii) the proposed GradTrust is in the Top-2 performing methods on $37$ of the considered $38$ experimental modalities. The code is available at: https://github.com/olivesgatech/GradTrust

==> Sections/3_Theory.tex <==
\section{Information in Counterfactual Gradients}
\label{sec:Theory}
Let $f(]cdot)$ be an $L$ layered neural network trained to distinguish between $N$ classes. If $x$ is any input to the network, the prediction from a classification application is given by $f(x) = y_l$ where $y_l$ is a $(N\times 1)$ vector of logits. The prediction $y$ is the index of the maxima of $y_l$. Consider only the final fully connected layer $f_{L}(\cdot)$ parameterized by weights ($W_L$) and bias ($b_L$). We obtain $y$ as,
\begin{equation}\label{eq:Filter}
\begin{gathered}
    y = W_L^T f_{L-1}(x) + b_L, \\
    \forall  y\in \Re^{N\times 1}, W_L\in \Re^{d_{L-1}\times N}, f_{L-1}(x)\in \Re^{d_{L-1}\times 1},
\end{gathered}
\end{equation}
where $f_{L-1}(x)$ is the flattened output of the network just before the final fully connected layer. The goal of training is construct $f_{L-1}(X)$ to span a linearly separable representation space so that $f_L(\cdot)$ can classify $x$ among $N$ classes via linear projection. However, this is rarely the case. On ImageNet~\cite{deng2009imagenet}, pretrained state-of-the-art PyTorch transformer architectures obtain a Top-1 accuracy of $82.7\%$. In this paper, we provide an accompanying reliability measure $r_x$ for a given prediction $y$ at inference.

At inference, we are provided with $f(\cdot)$ and $x$ only. Fisher information is the measure of information an observation $x$ yields regarding the underlying distribution $f_{L-1}(X)$ where $X$ is the training set. Note that we do not have access to $X$ at inference. We assume that $f_{L-1}(X)$ is a zero-mean $d_{L-1}$ dimensional multivariate gaussian distribution. Since large-scale neural networks consist of batch norm layers, this is generally a safe assumption. We estimate the reliability of a prediction $y$ as the ratio of Fisher information of the predicted class against the Fisher information of all counterfactual classes.  

Computationally, it is the variance of the score, or the expected value of the observed information. 

Let the output of the neural network be $f(x|W)$. The fisher information is given by,
\begin{equation}\label{eq:Fisher}
    I(W) = Var_{W}\bigg[\frac{d}{dW}l(x|W)\bigg],
\end{equation}
where $l(x|W)$ is some likelihood function. Mean square error quantifies the variance of error that is normally distributed. The log-likelihood is a function of MSE and some constants. Since Eq.~\ref{eq:Fisher} requires the derivative of the log-likelihood, we can ignore the constants and obtain the fisher information as, 
\begin{equation}\label{eq:Fisher_MSE}
    I(W) = Var_{W}\bigg[\frac{d}{dW}\text{MSE}_W(x,x')\bigg],
\end{equation}
Under normal distribution settings, minimizing Mean Square Error is the same as maximizing the Likelihood Estimate. 

Condider the output 




